Physics-Informed Neural Network for Multirotor Slung Load Systems Modeling

Recent advances in aerial robotics have enabled the use of multirotor vehicles for autonomous payload transportation. Resorting only to classical methods to reliably model a quadrotor carrying a cable-slung load poses significant challenges. On the other hand, purely data-driven learning methods do not comply by design with the problem's physical constraints, especially in states that are not densely represented in training data. In this work, we explore the use of physics informed neural networks to learn an end-to-end model of the multirotor-slung-load system and, at a given time, estimate a sequence of the future system states. An LSTM encoder decoder with an attention mechanism is used to capture the dynamics of the system. To guarantee the cohesiveness between the multiple predicted states of the system, we propose the use of a physics-based term in the loss function, which includes a discretized physical model derived from first principles together with slack variables that allow for a small mismatch between expected and predicted values. To train the model, a dataset using a real-world quadrotor carrying a slung load was curated and is made available. Prediction results are presented and corroborate the feasibility of the approach. The proposed method outperforms both the first principles physical model and a comparable neural network model trained without the physics regularization proposed.

==> complete_bib.tex <==
@article{sindy,
    author = {Steven L. Brunton and Joshua L. Proctor and J. Nathan Kutz},
    title = {Discovering governing equations from data by sparse identification of nonlinear dynamical systems},
    journal = {Proceedings of the National Academy of Sciences},
    volume = {113},
    number = {15},
    pages = {3932-3937},
    year = {2016},
    doi = {10.1073/pnas.1517384113}
}

@article{sindy_nn,
    author = {Kathleen Champion and Bethany Lusch and J. Nathan Kutz and Steven L. Brunton},
    title = {Data-driven discovery of coordinates and governing equations},
    journal = {Proceedings of the National Academy of Sciences},
    volume = {116},
    number = {45},
    pages = {22445-22451},
    year = {2019},
    doi = {10.1073/pnas.1906995116}
}

@article{PINNs,
    title = {Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations},
    journal = {Journal of Computational Physics},
    volume = {378},
    pages = {686-707},
    year = {2019},
    issn = {0021-9991},
    doi = {https://doi.org/10.1016/j.jcp.2018.10.045},
    author = {M. Raissi and P. Perdikaris and G.E. Karniadakis},
    keywords = {Data-driven scientific computing, Machine learning, Predictive modeling, Runge–Kutta methods, Nonlinear dynamics}
}

@book{thuerey2021pbdl,
  title={Physics-based Deep Learning},
  author={Nils Thuerey and Philipp Holl and Maximilian Mueller and Patrick Schnell and Felix Trost and Kiwon Um},
  url={https://physicsbaseddeeplearning.org},
  year={2021},
  publisher={WWW}
}

@article{pinns_mpc_robotic_arm,
    title = {Physics-informed Neural Networks-based Model Predictive Control for Multi-link Manipulators},
    journal = {IFAC-PapersOnLine},
    volume = {55},
    number = {20},
    pages = {331-336},
    year = {2022},
    note = {10th Vienna International Conference on Mathematical Modelling MATHMOD 2022},
    issn = {2405-8963},
    doi = {https://doi.org/10.1016/j.ifacol.2022.09.117},
    author = {Jonas Nicodemus and Jonas Kneifl and Jörg Fehr and Benjamin Unger},
    keywords = {Physics-informed Machine Learning, Model Predictive Control, Surrogate Model, Mechanical System, Real-time Control}
}

@article{Yu2023,
  title={Adaptive control with unknown mass estimation for a quadrotor-slung-load system},
  author={Yu, Gan and Xie, Wei and Cabecinhas, David and Cunha, Rita and Silvestre, Carlos},
  journal={{ISA Transactions}},
  volume={133},
  pages={412--423},
  year={2023},
  publisher={Elsevier}
}

@ARTICLE{example_kumar,
  author={Kan, Xinyue and Thomas, Justin and Teng, Hanzhe and Tanner, Herbert G. and Kumar, Vijay and Karydis, Konstantinos},
  journal={IEEE Robotics and Automation Letters}, 
  title={Analysis of Ground Effect for Small-Scale UAVs in Forward Flight}, 
  year={2019},
  volume={4},
  number={4},
  pages={3860-3867},
  doi={10.1109/LRA.2019.2929993}
}


==> sections/06_future_work.tex <==
% \section{Future Work}
%\label{sec:future_work}
% A pertinent line for 

% To train and validate the model designed, observations of state variables and control inputs $\{\vect{x}_k, \vect{u}_k \}$ were acquired from real-world flights. Given these observations, the model recursively predicts the evolution of the state of the quadrotor-slung-load system for $\mathrm{N}$ time steps, provided that the control inputs that were applied to the actual vehicle at those $\mathrm{N}$ time steps are fed to the decoder.

% To render the proposed model suitable for a larger domain of control applications, a pertinent line of research to follow is to extend the model so that it is able to predict the evolution of the system online. In this case, the system has access to past observations of state variables and control inputs, however, observations of future control inputs are not available. We thus propose combining our model with a control policy, obtained through reinforcement learning by having the real system interact with the environment, that is responsible for providing sequences of estimates of subsequent control inputs to the model presented in this work. A schematic that illustrates this approach is in Figure~\ref{fig:future_work}.


%In particular, a possible follow-up to this work would be to control the system presented so that it could follow a desired trajectory, for instance in the context of payload delivery. As stated, a control law for such a system  

%To follow-up of this sub-project to consider a Deep Deterministic Policy Gradient (DDPG) reinforcement learning, which is a model-free, online, off-policy reinforcement learning method.
%https://www.mathworks.com/help/reinforcement-learning/ug/ddpg-agents.html

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/future_work.pdf}
%     \caption{Possible future work approach. The model learned using the approach presented in this paper is combined with a control policy obtained through reinforcement learning by having the real system interact with the environment, using the learned dynamics model as a reference for the real system.}
%     \label{fig:future_work}
% \end{figure}

% ----------------------------------

==> sections/08_references.tex <==
\begin{thebibliography}{00}

\bibitem{simpkins2012system}
Alex Simpkins.
\textit{System identification: Theory for the user, (ljung, l.; 1999)[on the shelf]}.
\textit{IEEE Robotics \& Automation Magazine}, 19(2):95-96, 2012.
Publisher: IEEE.

\bibitem{soderstrom1989system}
Torsten Söderström and Petre Stoica.
\textit{System identification}.
Publisher: Prentice-Hall International, 1989.

\bibitem{van2012subspace}
Peter Van Overschee and B. De Moor.
\textit{Subspace identification for linear systems: Theory—Implementation—Applications}.
Publisher: Springer Science \& Business Media, 2012.


\bibitem{sindy_nn}
Kathleen Champion, Bethany Lusch, J. Nathan Kutz, and Steven L. Brunton.
\textit{Data-driven discovery of coordinates and governing equations}.
\textit{Proceedings of the National Academy of Sciences}, 116(45):22445-22451, 2019.
doi: 10.1073/pnas.1906995116.

\bibitem{PINNs}
M. Raissi, P. Perdikaris, and G.E. Karniadakis.
\textit{Physics-informed neural networks: A deep learning framework for solving forward and inverse problems involving nonlinear partial differential equations}.
\textit{Journal of Computational Physics}, 378:686-707, 2019.
doi: 10.1016/j.jcp.2018.10.045.


\bibitem{PINN_control_antonelo}
Eric Aislan Antonelo, Eduardo Camponogara, Laio Oriel Seman, Eduardo Rehbein de Souza, Jean Panaioti Jordanou, and Jomi F. Hübner.
\textit{Physics-Informed Neural Nets-based Control}.
\textit{CoRR}, abs/2104.02556, 2021.
URL: \url{https://arxiv.org/abs/2104.02556}.

\bibitem{pinns_mpc_robotic_arm}
Jonas Nicodemus, Jonas Kneifl, Jörg Fehr, and Benjamin Unger.
\textit{Physics-informed Neural Networks-based Model Predictive Control for Multi-link Manipulators}.
\textit{IFAC-PapersOnLine}, 55(20):331-336, 2022.
Note: 10th Vienna International Conference on Mathematical Modelling MATHMOD 2022.
doi: 10.1016/j.ifacol.2022.09.117.

\bibitem{Gedon_DeepStateSpace}
Daniel Gedon, Niklas Wahlström, Thomas B. Schön, and Lennart Ljung.
\textit{Deep State Space Models for Nonlinear System Identification}.
\textit{IFAC-PapersOnLine}, 54(7):481-486, 2021.
Note: 19th IFAC Symposium on System Identification SYSID 2021.
doi: 10.1016/j.ifacol.2021.08.406.



\bibitem{sindy}
Steven L. Brunton, Joshua L. Proctor, and J. Nathan Kutz.
\textit{Discovering governing equations from data by sparse identification of nonlinear dynamical systems}.
\textit{Proceedings of the National Academy of Sciences}, 113(15):3932-3937, 2016.
doi: 10.1073/pnas.1517384113.

\bibitem{thuerey2021pbdl}
Nils Thuerey, Philipp Holl, Maximilian Mueller, Patrick Schnell, Felix Trost, and Kiwon Um.
\textit{Physics-based Deep Learning}.
URL: \url{https://physicsbaseddeeplearning.org}.
Publisher: WWW, 2021.



\bibitem{Yu2023}
Gan Yu, Wei Xie, David Cabecinhas, Rita Cunha, and Carlos Silvestre.
\textit{Adaptive control with unknown mass estimation for a quadrotor-slung-load system}.
\textit{ISA Transactions}, 133:412-423, 2023.
Publisher: Elsevier.

\bibitem{example_kumar}
Xinyue Kan, Justin Thomas, Hanzhe Teng, Herbert G. Tanner, Vijay Kumar, and Konstantinos Karydis.
\textit{Analysis of Ground Effect for Small-Scale UAVs in Forward Flight}.
\textit{IEEE Robotics and Automation Letters}, 4(4):3860-3867, 2019.
doi: 10.1109/LRA.2019.2929993.

\bibitem{Kingma2014}
Diederik P. Kingma and Jimmy Ba.
\textit{Adam: A method for stochastic optimization}.
\textit{arXiv preprint arXiv:1412.6980}, 2014.

\bibitem{Bahdanau2014}
Dzmitry Bahdanau, Kyunghyun Cho, and Yoshua Bengio.
\textit{Neural Machine Translation by Jointly Learning to Align and Translate}.
\textit{arXiv preprint arXiv:1409.0473}, 2014.

\bibitem{pegasus}
Marcelo Jacinto, Joao Pinto, Jay Patrikar, John Keller, Rita Cunha, Sebastian Scherer, and Antonio Pascoal.
\textit{Pegasus Simulator: An Isaac Sim Framework for Multiple Aerial Vehicles Simulation}.
\textit{arXiv preprint arXiv:2307.05263}, 2023.

\bibitem{zhou2019continuity}
Yi Zhou, Connelly Barnes, Jingwan Lu, Jimei Yang, and Hao Li.
\textit{On the continuity of rotation representations in neural networks}.
In \textit{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 5745-5753, 2019.


\end{thebibliography}

==> sections/A_attachment.tex <==
%\section*{Appendix}
\vspace{-2ex}
\label{section:appendix}
\begin{table}[H]
    \centering
    % \renewcommand{\arraystretch}{1.2}
    \caption{Network architecture, trained using the hyperparameters $\lambda_1=\lambda_2=\lambda_3=\lambda_4=20$, $\phi=5$, $\psi=10$, $\rho=0.1$.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c}
    Layer Type & Output shape & \# Trainable Parameters\\
    \hline
    \hline
    Dense Layer 1 (with GELU activation) & 100 & 1 800\\
    \hline
    Dense Layer 2 (with GELU activation) & 200 & 20 200\\
    \hline 
    Dense Layer 3 (with GELU activation) & 300 & 60 300\\
    \hline 
    LSTM encoder with 3 layers & 20 & 32 480 \\
    \hline
    LSTM decoder with 3 layers and attention & 20 & 34 900 \\
    \hline
    Dense Layer 4 & 300 & 6 300\\
	\hline
    Dense Layer 5 (with GELU activation) & 200 & 60 200\\
	\hline
    Dense Layer 6 (with GELU activation) & 100 & 20 100\\
	\hline
    Dense Layer 7 & 26 & 2 626\\
    \hline
    \end{tabular}
    }
    \newline
    \\ \textbf{Total number of parameters}: 238 906
    \label{tab:network_architecture}
\end{table}

% \begin{table}[H]
%     \centering
%     \caption{Loss Hyperparameters.}
%     \begin{tabular}{c|c}
%     Parameter & Value\\
%     \hline 
%     \hline
%     $\lambda_1$ & 3\\    $\lambda_2$ & 1\\
%     $\lambda_3$ & 1\\
%     $\lambda_4$ & 2\\
%     \hline
%     $\phi_1, \phi_2, \phi_3$ & 5\\
%     \hline
%     $\psi_1$ & 2\\
%     \hline
%     $\rho_1$ & 2\\
%     $\rho_2$ & 1\\
%     \hline    
%     \end{tabular}    
%     \label{tab:loss_hyperparameters}
% \end{table}


% \begin{table}
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Inference time}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{ c|c|c|c|c|c } 
%     \hline
%     \multicolumn{2}{c|}{Horizon} & \multicolumn{2}{c|}{RTX3090} & \multicolumn{2}{c}{Jetson Orin Nano} \\
%     \hline
%     $M$ & $N$ & mean (ms) & std dev (ms) & mean (ms) & std dev (ms)\\ 
%     \hline
%     50 & 25 & 10.76 & 0.53 & 59.44 & 0.26 \\
%     % \hline
%     50 & 50 & 21.24 & 0.99 & 115.26 & 0.59\\
%     % \hline
%     25 & 50 & 22.19 & 1.15 & 121.95 & 0.41\\   
%     \hline
%     \end{tabular}}
%     \label{tab:inference_time}
% \end{table}

==> sections/data.tex <==
\section*{Data Acquisition}
To train our models, we are going to start by resorting to high-fidelity physics simulators such as NVIDIA Isaac Sim with the Pegasus \cite{pegasus} extension and NVIDIA Warp. The use of physical simulators allows to collect timeseries of the state of the agent, composed of a multirotor coupled with a tether to a payload, and then determine the differential equations that govern its evolution over time. The relevant states to collect are the position, linear velocity, and attitude (orientation and angular rates) of the quadrotor as well as the position and velocity of the slung load. Additionally, we plan to perform experiments at the indoor flying arena -- equipped with a motion capture (MOCAP) system -- at the Taguspark campus to collect a smaller dataset from real flight data. The datasets collected -- in simulation and real-world environments -- are going to be used to generate training, validation, and test sets. 

%-------------------------------------------------
% To train our models, we are going to start by resorting to high-fidelity physics simulators such as NVIDIA Isaac Sim with the Pegasus extension or NVIDIA War pto collect time series data of the state of the system composed of a multirotor coupled with a tether and a payload performing several flight maneuvers.

%\jpg{Tendo em conta o debate de hoje de manha, refraseva para To train our models, we are going to start by resorting to high-fidelity physics simulators such as NVIDIA Isaac Sim with the Pegasus extension and NVIDIA Warp. The use of physical simulators allow the agent, composed of a multirotor coupled with a tether to a payload, to interact with the environment, in order to obtain the system dynamics. (a ideia é dar a entender que os dados são gerados pelo agente em tempo real, pq é a questao que estavamos a discutir de "como é qd a previsao estiver mt fora". Isto vai na linha da descricao de um sistema com reinforcement learning, mas nao obrigatoriamente)} 
%-------------------------------------------------

The data obtained via simulation is going to be used to pre-train our model for single-step and/or multi-step prediction of the evolution of the state of the complete nonlinear system. Provided that satisfactory results have been obtained in the simulation environment, we intend to use the smaller training set obtained from real flight data to fine-tune the pre-trained model, allowing for sim-to-real transfer.

% \jpg{The data obtained via simulation is going to be used to pre-train our model for single-step and/or multi-step prediction of the evolution of the state of the complete nonlinear system. Provided that satisfactory results have been obtained in the simulation environment, we intend to use the smaller training set obtained from real flight data to fine-tune (em vez de refine, a matla do deeo usa o finetune) the pre-trained model, allowing for sim-to-real transfer.}


% -------------------------------------------------------------------------
% Pre-trained network in a realistic simulation environment
% Acquire real data and partion samples into training, validation, and test sets
% Multi-set prediction using the learned models?
% -------------------------------------------------------------------------

% -------------------------------------------------------------------------
% ${\bf{p}} = \begin{matrix} [x & y & z]^\top \end{matrix} \in \mathbb{R}^3$
% -------------------------------------------------------------------------
%\jpg{Elaborar sobre a data usada, nomeadamente estado do sistema}

%  a diverse set of rigid bodies
% from the simulation and MOCAP system

% as well as known parameters such as the mass of the vehicle and thrust curve. \st{These time series should contain the input given to the system over time as well as the vehicle's and payload position, orientation and velocity}. We also aim to collect real flight data from a quadrotor flying in an indoor arena equipped with a Motion Capture system located at the Taguspark campus. \jp{Acho que assumimos que sobre o veículo se sabe tudo. Quanto à carga e à corda, acho que podemos considerar que alguns dos seus parâmetros são desconhecidos.} 

% \todo[author=JP, color=green]{Tem-se conhecimento dos parâmetros físicos da load?}

% \todo[author=GS, color=orange, inline]{Em resposta ao Pinto: Diria que seria suposto isto estimar isso juntamente com o modelo em si. Talvez esteja a interpretar mal o que esta estrutura pinn+sindy consegue fazer.}

%We will be training neural networks using data generated by high-fidelity physics simulators, such as NVIDIA IsaacSim with the Pegasus extension or NVIDIA Warp. We also aim to learn the dynamics using real flight data collected from a quadrotor. To this end, we plan to use the Motion Capture system available at the indoor flying arena located in the Taguspark campus. 

% The relevant states to collect from the experimental apparatus are the position ${\bf{x}} = [x,y,z]^T \in \mathbb{R}^3$, attitude and velocity of the quadrotor as well as the position and velocity of the payload.

==> sections/description.tex <==
\section*{Project Description}

%The fascinating advancements in aerial robotics and associated fields of study have enabled the use of multirotor vehicles for payload transportation to become a reality. Many logistics and e-commerce enterprises have approached the aerial transportation problem by using small-scaled unmanned rotorcraft to carry packages attached to their body. The research community has extensively studied multirotor slung load systems composed of one or multiple aircraft. 
%---------------------------------------------

The fascinating advancements in aerial robotics have enabled the use of multirotor vehicles for payload transportation to become a reality. However, having a multirotor carrying a slung load attached by a string is still a challenge  -- for the intricate modeling of the system dynamics and the design of suitable tracking controllers. Resorting to data-driven techniques to learn the differential equations that govern a dynamical system is a promising strategy to address such difficulties. In this project, we aim to explore the combination of Physics-informed Neural Networks (PINNs)~\cite{PINNs} and the Sparse Identification of Nonlinear Dynamics (SINDy) framework~\cite{sindy,sindy_nn} to model the complex nonlinear interactions between a slung load and a multirotor vehicle (Figure \ref{fig:project_description}), and to estimate unknown physical parameters of the load.

% Place an image here
\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/payload.png}
    \caption{Graphical representation of the nonlinear system composed of a slung load and a multirotor.}
    \label{fig:project_description}
\end{figure}

% ---------- Removed/Improved by Joao Pinto -----------------
% \st{On the other hand The use of deep-learning techniques for dynamical modelling and low-level vehicle control is not widely adopted due to its inability to provide model explainability and stability guarantees, respectively}.   \todo[author=MJ,color=orange]{Estes parágrafos estão mesmo maus, mas vou melhorando à medida que as ideias ficam mais claras.}
% \st{deep-learning} 
% \st{leverage the use of mechanical cables/tethers} 
% \st{We will try to preserve the information known a priori of the model of a quadrotor and determine the governing state-space equations that describe the complex nonlinear interactions between the payload and the vehicle}. 

==> sections/evaluation_metrics.tex <==
\section*{Model Testing and Evaluation Metrics}

% As a first step to evaluate the validity of the learned dynamical models that expresses the interactions between a slung load and a multirotor vehicle
% -------------------------------

%As a first step to evaluating the validity of the learned dynamical models, we will be resorting to a realistic simulation environment. Provided that satisfactory simulation results have been obtained, we intend to conduct further experimental trials at the indoor flying arena previously mentioned.

% in the indoor flying arena previously mentioned to further validate the proposed approach. 

For evaluation metrics, we will be considering: i) computation speed; and ii) tracking performance. As such, we are going to resort to metrics such as root-mean-square error (RMSE) of the positions and orientations of both the multirotor and the load -- in the simulation and real-world environments -- to compare the output predictions of the models with the simulation and real test sets. 

% -------------------------------
% \jpg{Nao estou habitado ao uso de PSNR neste contexto, por isso se calhar tirava, e metoa no relatorio final se virmos que faz sentido.}
% -------------------------------

We are also aiming to compare the algorithm that we will have designed with strategies proposed in the literature that consider dynamical models solely obtained from first principles and adaptive controllers with online estimation of the unknown parameters of the slung load, for instance, the recent work of Yu et al.~\cite{Yu2023}. 

% Finally, we contemplate drawing some conclusions on the stability of the multirotor slung load system in closed-loop with one of the controllers we will have implemented if time allows.

% -------------------------------

% \todo[author=JP,color=green,inline]{Fiz o melhor possível para sintetizar o texto da versão anterior da proposta. Por enquanto, não me atrevo a alterar/cortar mais texto para que todas as secções fiquem contidas numa única página. A meu ver, as secções "Methodology" e "Model Testing and Evaluation Metrics" são aquelas que mais facilmente podem ser encortadas/reformuladas. Também já reduzi ligeiramente o espaçamento entre parágrafos para o texto ficar mais compacto. Bom trabalho!}

% -------------------------------
% Our proposed algorithms are going to be compared with current approaches based on: i) computation speed; ii) tracking performance; and iii) stability and ability to recover. We mean to test the approaches in a \texthl{realistic} simulation environment -- considering reference trajectories not present in the training set -- and using a drone flying in the indoor arena \texthl{or an actual inverted pendulum}, should everything go according to plan. 

% \todo[author=MJ, color=orange]{Isto ainda faz sentido, tendo em conta que já não vamos falar de controladores neste projeto?}

% -------------------------------
%\todo[author=JP,color=cyan,inline]{Por mim, ficaria assim. Talvez seja melhor que as conclusões sobre a estabilidade do sistema fiquem de fora.}

% \st{performance of the proposed algorithms}
% \st{We will attempt to apply the suggested control strategy to stabilize a double integrator system, followed by an inverted pendulum, and then a quadrotor.}

% In order to evaluate the performance of the proposed algorithms, we will be resorting to the simulation of dynamical systems with growing levels of complexity. First, we will attempt to apply the suggested control strategy to stabilize a double integrator system, followed by an inverted pendulum and a quadrotor. \st{To gather training data, we will rely mostly on a}
%\jpg{Acho que aqui estamos a misturar as coisas. O data é mais training data, e não tt para avaliar a performance. Esta descrição é mais evaluation metrics. Fiz umas alterações, caso concordem, para separar em duas secções.}
% In order to evaluate the performance of the proposed algorithms, 
%\jpg{Podemos cortar o real}
%\jpg{As duas primeiras parecem ok, a 3a era para analisarmos regioes de convergencia por alto, nao sei se faz sentido.}
%\jp{Concordo, podemos falar de estabilidade, mas num sentido mais lato... É mais perceber em que condições o sistema funciona de forma empírica, diria eu. Para o tempo que temos, regiões de convergência, não.}
%\todo[author=JP,color=cyan,inline]{Já que na descrição do projeto estabelecemos como objetivo estimar a dinâmica da interação entre o drone e a slung load, a principal meta de avaliação é ter um multirotor com uma corda a segurar uma carga e -- tanto o multirotor como a carga -- descreverem as trajetórias pretendidas. Se tudo correr bem em ambiente simulação é que se avança para ensaios experimentais, a meu ver.}
%\todo[author=JP,color=cyan,inline]{Diria que o inverted pendulum e double integrators são fallback plans.}

==> sections/methodology.tex <==
\section*{Methodology}

%---------------------------------------------
% Original paragraph written by MJ
% PINNs are neural networks that are trained using supervised learning methods to approximate the nonlinear parameterized partial differential equations (PDE)s or ordinary differential equations (ODE)s of the form

% \begin{equation}
%     \frac{\partial u}{\partial t} + \mathcal{N}[u; \lambda] = 0 , ~ x \in \Omega, ~ t \in [0, T],
% \end{equation}

% where $u(t, x)$ is the latent solution which should be approximated by a deep neural network, $\mathcal{N}[\cdot; \lambda]$ is a differential operator -- parameterized by $\lambda$ -- and $\Omega$ a subset of $\mathbb{R}^{N}$. \st{ where $N$ denotes the dimension of the system}. Their goal is, given the current time $t$ and state of a dynamical system $x$, predict the derivative of the system state $\partial u(t, x) / \partial t$.
%---------------------------------------------

Given measurements of the spatio-temporal evolution of a system described by a nonlinear partial differential equation of the form, $\partial_t u + \mathcal{N}[u; \lambda] = 0$, where $\mathcal{N}[\hspace{.2ex}\cdot\hspace{.2ex}; \lambda]$ corresponds to a differential operator parameterized by $\lambda$, PINNs -- neural networks that are trained to solve supervised learning tasks while taking into account the system dynamics -- can provide an estimate of the parameters $\lambda$ that best describes the observed data~\cite{PINNs}. 

% This is achieved by considering a loss function that enforces the structure of the dynamics at a finite set of collocation points drawn from the admissible spatio-temporal domain.

%---------------------------------------------
% M. Raissi et al., "Physics-informed neural networks", 2019
% 
% "One potential limitation of the continuous time neural network models considered so far stems from the need to use a large number of collocation points $N_f$ in order to enforce physics-informed constraints in the entire spatio-temporal domain. Although this poses no significant issues for problems in one or two spatial dimensions, it may introduce a severe bottleneck in higher dimensional problems ... we put forth a different approach that circumvents the need for collocation points by introducing a more structured neural network representation leveraging the classical Runge–Kutta time-stepping schemes"
%--------------------------------------------- 

Although standard PINN models are extremely useful in a variety of physics problems, they hinge on the knowledge of the differential operator $\mathcal{N}$. For instance, in the application being considered -- a multirotor vehicle carrying a slung load attached by a string -- under the assumption that the string is taut, the dynamics of the complete system can be derived from first principles. Dropping this simplifying assumption renders the problem of deriving the dynamics hard.

%---------------------------------------------
% Original paragraph written by MJ
% Alternative models -- such as SINDy -- exploit the idea of a "bag of functions" to propose a method for the discovery of functions that govern the dynamics of physical phenomena, based on a formulation of a convex sparse linear regression problem using a linear combination of nonlinear functions. This model falls short when the dynamics of the system cannot be expressed by a combination of function in the "bag of functions" and the observable state variables. An extension of SINDy proposes the combination of this algorithm with a neural network (NN) with an autoencoder structure \citep{sindy_nn} to simultaneously discover a low-dimensional latent space of coordinates and functions that model the dynamics of the system in that latent space. To achieve this, the SINDy loss is incorporated in the NN loss as a part of the training. 
%---------------------------------------------

Alternative models -- such as SINDy -- propose expressing the dynamics, given by ordinary differential equations (ODEs), as a linear combination of nonlinear basis functions. To determine the contribution of each basis function, a convex sparse linear regression problem is formulated~\cite{sindy}. An extension of SINDy proposes the combination of this algorithm with a neural network (NN) with an autoencoder structure to simultaneously discover a low-dimensional latent space of coordinates and functions that model the dynamics of the system in that low-dimensional space~\cite{sindy_nn}. 

% To achieve this, the SINDy loss is incorporated in the NN loss as a part of the training. 

In this work, we plan to combine the PINN and NN-SINDy models and extend them to dynamical systems, described by ODEs, with a forced regime. Leveraging the literature on the design of controllers for multirotor slung load systems, we intend to implement an existing one with the added novelty of using the learned model for the system dynamics of the combined rotorcraft and load. 

% \jpg{refraseava isto, o que acham de Leveraging the literature on the design of controllers for multirotor slung load systems, we intend to implement an existing controller, . }

%---------------------------------------------
% i.e. dynamical systems with inputs of the form 
% \begin{equation}
%     \frac{d x}{d t} = f(x, t, u; \lambda),
% \end{equation}
% where $x$ denotes the state of the system, $t$ the time , $u$ is the system input and $\lambda$ are parametric values. This strategy will allow for the training of a network while exploiting the equations that describe the multirotor dynamics which are well described in the literature while at the same time discovering a latent space and a set of equations that can be used to model the slung-load system coupled to the aircraft. Such model could then be theoretically incorporated in a control strategy such as Model Predictive Control (MPC).
